StructRAG: Boosting Knowledge Intensive Reasoning of LLMs via Inference-time Hybrid Information Structurization

Retrieval-augmented generation (RAG) is a key means to effectively enhance large language models (LLMs) in many knowledge-based tasks. However, existing RAG methods struggle with knowledge-intensive reasoning tasks, because useful information required to these tasks are badly scattered. This characteristic makes it difficult for existing RAG methods to accurately identify key information and perform global reasoning with such noisy augmentation. In this paper, motivated by the cognitive theories that humans convert raw information into various structured knowledge when tackling knowledge-intensive reasoning, we proposes a new framework, StructRAG, which can identify the optimal structure type for the task at hand, reconstruct original documents into this structured format, and infer answers based on the resulting structure. Extensive experiments across various knowledge-intensive tasks show that StructRAG achieves state-of-the-art performance, particularly excelling in challenging scenarios, demonstrating its potential as an effective solution for enhancing LLMs in complex real-world applications.

==> figures/head.tex <==
% \begin{figure}[t]
% \centering
% \includegraphics[width=\linewidth]{figures/head_fig_h.pdf} 
% \caption{In contrast to existing RAG and Graph RAG methods, our StructRAG constructs and utilizes the most suitable structured knowledge, effectively addressing diverse knowledge-intensive reasoning tasks.} 
% \label{fig:domain}
% \end{figure}

\begin{wrapfigure}{r}{0.45\textwidth}
\vspace{-0.5cm}{\includegraphics[width=65mm]{figures/head_fig.pdf}
\vspace{-0.3cm}
\caption{In contrast to existing RAG and Graph RAG methods, our StructRAG constructs and utilizes the most suitable structured knowledge, effectively addressing diverse knowledge-intensive reasoning tasks.}
\label{fig:domain}
}
\end{wrapfigure}

==> figures/router.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=0.48\linewidth]{figures/router_fig.pdf} 
\caption{Scores and exact matching rate of StructRAG with different routers. The figure shows that stronger router can have positive impact on the final performance of StructRAG framework.} 
\label{fig:router}
\end{figure}

==> tables/ablation.tex <==
\begin{table*}[t]
\centering  
\resizebox{\textwidth}{!}{
\begin{tabular}{l|cccc}
\toprule

\multirow{1}{*}{} & \multicolumn{1}{c}{Spotlight Locating} & \multicolumn{1}{c}{Comparison} & \multicolumn{1}{c}{Clustering} & \multicolumn{1}{c}{Chain of Reasoning} \\
\midrule
Ours & \textbf{66.70} & \textbf{57.40} & \textbf{42.43} & \textbf{56.64} \\ 
no agent & 63.40 & 50.92 & 40.10 & 50.18 \\ 
no structure & 59.41 & 51.41 & 40.76 & 48.16 \\ 
\bottomrule
\end{tabular}
}
\caption{The result of adding RAG module on Qwen2-72B-Instruct with different length sets. }
\label{tb:rag_qwen2}
\end{table*}


==> tables/case.tex <==
\begin{wraptable}{r}{0.5\textwidth}
\centering
\vspace{-0.4cm}
\resizebox{0.48\textwidth}{!}{
\begin{tabularx}{\columnwidth}{lX}
\toprule
\multirow{3}{*}{\textbf{Raw}} 
& 
Here is report of company A: In 2024, the payment is primarily consisted \\ 
& of a net loss of (including: depreciation of \textbf{\$ 1,308,463} and share-based  \\ 
& compensation expense of \textbf{\$ 537,197}) ... 
\\

\midrule
\multirow{1}{*}{\textbf{Structured}}
& 
\begin{minipage}[b]{0.7\columnwidth}
\centering
\raisebox{-.2\height}{\includegraphics[width=\columnwidth]{figures/case_fig.pdf}}
\end{minipage}
\\

\bottomrule
\end{tabularx}
}
\caption{Some cases to show why EM rate of StructRAG is not perfect. The reason is structurization may cause some textual difference.}
\label{table:case}
\end{wraptable}

==> tables/effeciency.tex <==
\begin{wraptable}{r}{0.5\textwidth}
\centering
\vspace{-0.4cm}
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{lccc}
\toprule
\textbf{Method}    & \textbf{Constructing} & \textbf{Reading} & \textbf{Total Latency} \\ 
\midrule
RQ-RAG~\citep{chan2024rqraglearningrefinequeries}  & 7.8   & 1.2 & 9.0           \\
GraphRAG~\citep{edge2024localglobalgraphrag}  &215.3 & 1.8 & 217.1 \\
StructRAG (Ours) &8.2 &1.5 &9.7         \\ 
\bottomrule
\end{tabular}
}
\vspace{-0.1cm}
\caption{Comparison of implementing latency (minute). The StructRAG has an available speed, which is much faster than GraphRAG.}
\label{table:effiency}
\end{wraptable}


==> tables/multiagent.tex <==
\begin{table}[t]
\resizebox{0.48\linewidth}{!}{
\begin{tabular}{lcccc}
\toprule
 & Spot. & Comp. & Clus. & Chain. \\
\midrule
\textbf{StructRAG} & \textbf{67.49} & \textbf{63.12} & \textbf{60.45} & \textbf{53.86} \\ 
~w/ 7B construction& 51.32 & 44.86 & 32.68 &38.23 \\ 
~w/ 7B analysis & 52.68 & 52.36 & 44.21 & 47.88 \\ 
~w/ 7B retrieval  & 45.45 & 46.39 & 51.65 & 48.23 \\ 
~w/ 7B merging  & 58.68 & 46.39 & 45.73 & 34.58 \\ 
\bottomrule
\end{tabular}
}
\caption{Results of replacing one agent to a 7B model. The table shows that construction agent is the most important part, and the importance sorting of agents varies in these four tasks.}
\label{table:multiagent}
\end{table}


==> tables/multiagent_and_case.tex <==
\begin{figure*}
    \begin{minipage}[t]{0.48\linewidth}
    \vspace{0pt}
    \centering
    \scriptsize
    \captionsetup{type=table} 
\resizebox{\columnwidth}{!}{
\begin{tabular}{lcccc}
\toprule
 & Spot. & Comp. & Clus. & Chain. \\
\midrule
\textbf{StructRAG} & \textbf{67.49} & \textbf{63.12} & \textbf{60.45} & \textbf{53.86} \\ 
~w/ 7B construction& 51.32 & 44.86 & 32.68 &38.23 \\ 
~w/ 7B analysis & 52.68 & 52.36 & 44.21 & 47.88 \\ 
~w/ 7B retrieval  & 45.45 & 46.39 & 51.65 & 48.23 \\ 
~w/ 7B merging  & 58.68 & 46.39 & 45.73 & 34.58 \\ 
\bottomrule
\end{tabular}
}
\caption{Results of replacing one agent to a 7B model. The table shows that construction agent is the most important part, and the importance sorting of agents varies in these four tasks.}
\label{table:multiagent}
    \end{minipage}
    \hfill % 分隔符
    \begin{minipage}[t]{0.48\linewidth}
    \vspace{0pt}
    \centering  
    % \tiny
    \scriptsize
    \captionsetup{type=table} 
% \resizebox{\columnwidth}{!}{
\begin{tabularx}{\columnwidth}{lX}
\toprule
Raw & 
Here is report of company A: In 2024, the payment is primarily consisted of a net loss of (including: depreciation of \textbf{\$ 1,308,463} and share-based compensation expense of \textbf{\$ 537,197}) ... \\
\midrule
Structured & 
\begin{minipage}[b]{0.7\columnwidth}
\centering
\raisebox{-.2\height}{\includegraphics[width=\linewidth]{figures/case_fig.pdf}}
\end{minipage}
\\
\bottomrule
\end{tabularx}
% }
\caption{Some cases to show why EM rate of StructRAG is not perfect. The reason is structurization process may cause a little difference in textual format of original documents.}
\label{table:case}
    \end{minipage}

\end{figure*}

==> tables/router.tex <==
\begin{table}[t]
\centering  
\resizebox{0.48\linewidth}{!}{
\begin{tabular}{lcc}
\toprule
 & F1 & ACC \\
\midrule
{Hybrid Structure Router} & \textbf{93.42} & \textbf{94.38} \\ 
Qwen2-7B-Instruct (zero-shot) & 50.04 & 54.25  \\ 
Qwen2-7B-Instruct (few-shot) & 65.59 & 66.12  \\ 
Qwen2-72B-Instruct (zero-shot) & 78.38 & 80.56  \\ 
Qwen2-72B-Instruct (few-shot) & 89.39 & 90.06  \\ 
\bottomrule
\end{tabular}
}
\caption{Results of evaluating knowledge preference routers. The table shows that preference training is necessary for the routing ability.}
\label{table:router}
\end{table}


==> tables/summary.tex <==
\begin{table*}[t]
\centering  
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccccccc}
\toprule
  
 & 
\multicolumn{2}{c}{Spot.} & 
\multicolumn{2}{c}{Comp.} & 
\multicolumn{2}{c}{Clus.} & 
\multicolumn{2}{c}{Chain.} & 
\multicolumn{2}{c}{Overall} \\ 

\cmidrule(lr){2-3} 
\cmidrule(lr){4-5}  
\cmidrule(lr){6-7}
\cmidrule(lr){8-9}
\cmidrule(lr){10-11}

 & 
Score  & 
EM Rate & 
Score  & 
EM Rate & 
Score  & 
EM Rate & 
Score  & 
EM Rate & 
Score  & 
EM Rate \\ 

\midrule

\rowcolor[rgb]{ .906,  .902,  .902}
\multicolumn{11}{c}{Set 1~~(10K-50K)} \\ 

\midrule

Long-context~\citep{yang2024qwen2technicalreport} & 68.49 & \textbf{0.55} & 60.60 & 0.37 & 47.08 & 0.08 & \textbf{70.39} & \textbf{0.36} & 60.11 & 0.29\\ 
% RAG Top-5~\citep{NEURIPS2020_6b493230}  &54.62 &0.45 &26.17 &0.08 &29.60 &0.03 &34.41 &0.08 &34.51 &0.12 \\
RAG~\citep{NEURIPS2020_6b493230}   &51.08 &0.35 &44.53 &0.27 &37.96 &0.05 &53.95 &0.35 &46.11 &0.23 \\
RQ-RAG~\citep{chan2024rqraglearningrefinequeries}   &70.60 & 0.48& 61.42& 0.38& 58.33& 0.12& & & & \\
GraphRAG~\citep{edge2024localglobalgraphrag}   & 48.12 & & & & & & & & & \\
\textbf{StructRAG}    & \textbf{74.53} & 0.47& \textbf{75.58} &  \textbf{0.47} & \textbf{65.13} & \textbf{0.23} & 67.84 &  0.34 & \textbf{69.43} & \textbf{0.35} \\
67

\bottomrule
\end{tabular}
}
\caption{Scores and exact matching rate in knowledge-intensive QA tasks. From Set 1 to Set 4, task complexity gradually increases, as reflected by the growing token number of documents. StructRAG get the SOTA performance in  overall metrics. And the more complex the task, the greater the improvement of StructRAG.}
\label{table:main_results}
\end{table*}

==> tables/tmp.tex <==
\begin{table*}[t]
\centering  
\resizebox{\textwidth}{!}{
\begin{tabular}{l|cc|cc|cc|cc|cc}
\toprule

\multirow{1}{*}{\textbf{Qwen2-72B-Instruct (128K)}} & \multicolumn{2}{c|}{\textbf{Spotlight Locating}} & \multicolumn{2}{c|}{\textbf{Comparison}} & \multicolumn{2}{c|}{\textbf{Clustering}} & \multicolumn{2}{c|}{\textbf{Chain of Reasoning}} & \multicolumn{2}{c}{\textbf{Overall}}\\
\midrule
\multicolumn{11}{c}{\textbf{ $\mathtt{Set1}$ (10K-50K)}} \\
Qwen2-72B-Instruct (128K) & 68.49 & 0.55 & 60.60 & 0.37 & 47.08 & 0.08 & 70.39 & 0.36 & 60.11 & 0.29\\ 
\textit{w/ Openai Embedding, Top k=5} &54.62 &0.45 &26.17 &0.08 &29.60 &0.03 &34.41 &0.08 &34.51 &0.12 \\
\textit{w/ BGE Embedding, Top k=5} & 62.92 &0.53 &30.92 &0.08 &31.28 &0.03 &32.95 &0.11 &36.91 &0.15 \\
\textit{w/ Openai Embedding, Top k=10} & 59.81 &0.43 &34.93 &0.15 &29.33 &0.02 &41.27 &0.15 &38.96 &0.15 \\
\textit{w/ BGE Embedding, Top k=10}& 72.13 &0.62 &32.42 &0.12 &31.90 &0.05 &44.12 &0.20 &42.27 &0.20 \\
\textit{w/ Openai Embedding, Top k=30}&57.26 &0.40 &45.43 &0.28 &40.04 &0.06 &57.32 &0.35 &49.06 &0.24 \\
\textit{w/ BGE Embedding, Top k=30}&56.37 &0.33 &46.27 &0.30 &38.35 &0.10 &51.49 &0.29 &46.69 &0.23 \\
\textit{w/ Openai Embedding, Top k=50} &51.08 &0.35 &44.53 &0.27 &37.96 &0.05 &53.95 &0.35 &46.11 &0.23 \\
\textit{w/ BGE Embedding, Top k=50}&53.47 &0.37 &47.31 &0.29 &36.42 &0.06 &54.65 &0.35 &46.62 &0.24 \\
\textbf{Ours}& 67.66&0.51 & \textbf{68.80} & \textbf{0.45} & \textbf{51.44} & \textbf{0.14} & \textbf{72.54} & \textbf{0.45} & \textbf{63.66} & \textbf{0.35} \\

\midrule
\multicolumn{11}{c}{\textbf{ $\mathtt{Set2}$ (50K-100K)}} \\
Qwen2-72B-Instruct (128K) & 64.53 & 0.43 & 42.60 & 0.21 & 38.52 & 0.05 & 51.18 & 0.20 & 45.71 & 0.17\\ 
\textit{w/ Openai Embedding, Top k=5} & 56.64 &0.40 &36.68 &0.19 &30.91 &0.03 &28.38 &0.01 &34.54 &0.10 \\
\textit{w/ BGE Embedding, Top k=5} &67.29 &0.47 &43.39 &0.28 &28.31 &0.03 &32.22 &0.07 &36.95 &0.14 \\
\textit{w/ Openai Embedding, Top k=10} & 67.07 &0.53 &44.30 &0.27 &34.31 &0.05 &34.03 &0.06 &40.17 &0.15 \\
\textit{w/ BGE Embedding, Top k=10}& 71.74 &0.54 &47.68 &0.30 &30.55 &0.03 &30.57 &0.03 &38.80 &0.14 \\
\textit{w/ Openai Embedding, Top k=30}&66.27 &0.46 &46.28 &0.31 &38.95 &0.05 &46.15 &0.22 &45.42 &0.19 \\
\textit{w/ BGE Embedding, Top k=30}&57.35 &0.41 &46.92 &0.29 &35.30 &0.05 &42.82 &0.20 &42.04 &0.18 \\
\textit{w/ Openai Embedding, Top k=50}&55.94 &0.32 &47.94 &0.31 &34.32 &0.03 &46.64 &0.21 &42.60 &0.16 \\
\textit{w/ BGE Embedding, Top k=50}&59.41 &0.39 &38.52 &0.21 &35.40 &0.06 &45.47 &0.24 &41.51 &0.17 \\
\textbf{Ours}& 66.87& \textbf{0.56} & \textbf{56.24} & \textbf{0.39} & \textbf{43.48} & \textbf{0.06} & \textbf{52.99} & \textbf{0.29} & \textbf{51.17} & \textbf{0.24} \\



\midrule
\multicolumn{11}{c}{\textbf{ $\mathtt{Set3}$ (100K-200K)}} \\
Qwen2-72B-Instruct (128K) & 46.99 & 0.27 & 37.06 & 0.13 & 31.50 & 0.02 & 35.01 & 0.07 & 35.94 & 0.09\\ 
\textit{w/ Openai Embedding, Top k=5} &63.91 &0.44 &33.56 &0.17 &25.98 &0.01 &28.98 &0.04 &34.48 &0.12 \\
\textit{w/ BGE Embedding, Top k=5} &64.81 &0.47 &30.27 &0.14 &25.88 &0.01 &27.86 &0.05 &33.70 &0.12 \\
\textit{w/ Openai Embedding, Top k=10} &67.50 &0.46 &33.44 &0.16 &27.94 &0.02 &31.62 &0.06 &36.47 &0.13 \\
\textit{w/ BGE Embedding, Top k=10}& 75.88 &0.56 &33.76 &0.15 &27.20 &0.01 &30.17 &0.04 &37.28 &0.14 \\
\textit{w/ Openai Embedding, Top k=30}&73.69 &0.55 &42.20 &0.27 &32.78 &0.02 &37.65 &0.13 &42.60 &0.18 \\
\textit{w/ BGE Embedding, Top k=30}&67.50 &0.47 &42.42 &0.18 &32.34 &0.03 &37.85 &0.12 &41.35 &0.15 \\
\textit{w/ Openai Embedding, Top k=50}&67.44 &0.50 &41.82 &0.24 &31.59 &0.04 &37.29 &0.12 &40.90 &0.18 \\
\textit{w/ BGE Embedding, Top k=50}&62.56 &0.42 &40.41 &0.18 &29.82 &0.02 &40.31 &0.14 &39.84 &0.15 \\
\textbf{Ours}& \textbf{76.73} & \textbf{0.63} & \textbf{55.41} & \textbf{0.38} & \textbf{39.68} & \textbf{0.05} & \textbf{47.51} & \textbf{0.22} & \textbf{50.66} & \textbf{0.25} \\


\midrule
\multicolumn{11}{c}{\textbf{$\mathtt{Set4}$ (200K-250K)}} \\
Qwen2-72B-Instruct (128K) & 33.18 & 0.16 & 26.59 & 0.08 & 29.84 & 0.01 & 25.81 & 0.04 & 28.92 & 0.06\\ 
\textit{w/ Openai Embedding, Top k=5} &51.49 &0.26 &17.12 &0.03 &21.59 &0.00 &16.37 &0.00 &25.59 &0.06 \\
\textit{w/ BGE Embedding, Top k=5} &48.40 &0.26 &14.55 &0.00 &20.69 &0.00 &18.07 &0.00 &24.63 &0.05 \\
\textit{w/ Openai Embedding, Top k=10} & 50.32 &0.28 &20.30 &0.03 &24.56 &0.00 &16.38 &0.00 &27.08 &0.06 \\
\textit{w/ BGE Embedding, Top k=10}& 51.02 &0.28 &21.88 &0.03 &25.45 &0.00 &17.29 &0.00 &28.10 &0.06 \\
\textit{w/ Openai Embedding, Top k=30}&52.17 &0.24 &24.60 &0.10 &26.78 &0.00 &17.79 &0.00 &29.29 &0.07 \\
\textit{w/ BGE Embedding, Top k=30}&47.98 &0.21 &26.82 &0.10 &26.70 &0.00 &20.02 &0.00 &29.44 &0.06 \\
\textit{w/ Openai Embedding, Top k=50}&51.63 &0.26 &23.62 &0.08 &24.49 &0.00 &21.84 &0.02 &29.14 &0.07 \\
\textit{w/ BGE Embedding, Top k=50}&47.23 &0.28 &27.78 &0.08 &26.48 &0.00 &24.44 &0.02 &30.52 &0.08 \\
\textbf{Ours}& \textbf{52.70}& \textbf{0.30}& \textbf{48.05}& \textbf{0.25}& \textbf{34.00}& \textbf{0.01}& \textbf{56.68}& \textbf{0.37}&\textbf{44.97} & \textbf{0.20}\\

\bottomrule
\end{tabular}
}
\caption{The result of adding RAG module on Qwen2-72B-Instruct with different length sets. }
\label{tb:rag_qwen2}
\end{table*}






\begin{table*}[t]
\centering  
\resizebox{\textwidth}{!}{
\begin{tabular}{l|cc|cc|cc|cc|cc}
\toprule

\multirow{1}{*}{\textbf{Qwen2-72B-Instruct (128K)}} & \multicolumn{2}{c|}{\textbf{Spotlight Locating}} & \multicolumn{2}{c|}{\textbf{Comparison}} & \multicolumn{2}{c|}{\textbf{Clustering}} & \multicolumn{2}{c|}{\textbf{Chain of Reasoning}} & \multicolumn{2}{c}{\textbf{Overall}}\\
\midrule
\multicolumn{11}{c}{\textbf{ $\mathtt{Set1}$ (10K-50K)}} \\
Qwen2-72B-Instruct (128K) & 68.49 & 0.55 & 60.60 & 0.37 & 47.08 & 0.08 & 70.39 & 0.36 & 60.11 & 0.29\\ 
\textit{w/ Openai Embedding, Top k=10} & 59.81 &0.43 &34.93 &0.15 &29.33 &0.02 &41.27 &0.15 &38.96 &0.15 \\
\textit{w/ BGE Embedding, Top k=10}& 72.13 &0.62 &32.42 &0.12 &31.90 &0.05 &44.12 &0.20 &42.27 &0.20 \\
\textit{w/ Openai Embedding, Top k=50} &51.08 &0.35 &44.53 &0.27 &37.96 &0.05 &53.95 &0.35 &46.11 &0.23 \\
\textit{w/ BGE Embedding, Top k=50}&53.47 &0.37 &47.31 &0.29 &36.42 &0.06 &54.65 &0.35 &46.62 &0.24 \\
\textbf{Ours}& 67.66&0.51 & \textbf{68.80} & \textbf{0.45} & \textbf{51.44} & \textbf{0.14} & \textbf{72.54} & \textbf{0.45} & \textbf{63.66} & \textbf{0.35} \\

\midrule
\multicolumn{11}{c}{\textbf{ $\mathtt{Set2}$ (50K-100K)}} \\
Qwen2-72B-Instruct (128K) & 64.53 & 0.43 & 42.60 & 0.21 & 38.52 & 0.05 & 51.18 & 0.20 & 45.71 & 0.17\\ 
\textit{w/ Openai Embedding, Top k=10} & 67.07 &0.53 &44.30 &0.27 &34.31 &0.05 &34.03 &0.06 &40.17 &0.15 \\
\textit{w/ BGE Embedding, Top k=10}& 71.74 &0.54 &47.68 &0.30 &30.55 &0.03 &30.57 &0.03 &38.80 &0.14 \\
\textit{w/ Openai Embedding, Top k=50}&55.94 &0.32 &47.94 &0.31 &34.32 &0.03 &46.64 &0.21 &42.60 &0.16 \\
\textit{w/ BGE Embedding, Top k=50}&59.41 &0.39 &38.52 &0.21 &35.40 &0.06 &45.47 &0.24 &41.51 &0.17 \\
\textbf{Ours}& 66.87& \textbf{0.56} & \textbf{56.24} & \textbf{0.39} & \textbf{43.48} & \textbf{0.06} & \textbf{52.99} & \textbf{0.29} & \textbf{51.17} & \textbf{0.24} \\



\midrule
\multicolumn{11}{c}{\textbf{ $\mathtt{Set3}$ (100K-200K)}} \\
Qwen2-72B-Instruct (128K) & 46.99 & 0.27 & 37.06 & 0.13 & 31.50 & 0.02 & 35.01 & 0.07 & 35.94 & 0.09\\ 
\textit{w/ Openai Embedding, Top k=10} &67.50 &0.46 &33.44 &0.16 &27.94 &0.02 &31.62 &0.06 &36.47 &0.13 \\
\textit{w/ BGE Embedding, Top k=10}& 75.88 &0.56 &33.76 &0.15 &27.20 &0.01 &30.17 &0.04 &37.28 &0.14 \\
\textit{w/ Openai Embedding, Top k=50}&67.44 &0.50 &41.82 &0.24 &31.59 &0.04 &37.29 &0.12 &40.90 &0.18 \\
\textit{w/ BGE Embedding, Top k=50}&62.56 &0.42 &40.41 &0.18 &29.82 &0.02 &40.31 &0.14 &39.84 &0.15 \\
\textbf{Ours}& \textbf{76.73} & \textbf{0.63} & \textbf{55.41} & \textbf{0.38} & \textbf{39.68} & \textbf{0.05} & \textbf{47.51} & \textbf{0.22} & \textbf{50.66} & \textbf{0.25} \\


\midrule
\multicolumn{11}{c}{\textbf{$\mathtt{Set4}$ (200K-250K)}} \\
Qwen2-72B-Instruct (128K) & 33.18 & 0.16 & 26.59 & 0.08 & 29.84 & 0.01 & 25.81 & 0.04 & 28.92 & 0.06\\ 
\textit{w/ Openai Embedding, Top k=10} & 50.32 &0.28 &20.30 &0.03 &24.56 &0.00 &16.38 &0.00 &27.08 &0.06 \\
\textit{w/ BGE Embedding, Top k=10}& 51.02 &0.28 &21.88 &0.03 &25.45 &0.00 &17.29 &0.00 &28.10 &0.06 \\
\textit{w/ Openai Embedding, Top k=50}&51.63 &0.26 &23.62 &0.08 &24.49 &0.00 &21.84 &0.02 &29.14 &0.07 \\
\textit{w/ BGE Embedding, Top k=50}&47.23 &0.28 &27.78 &0.08 &26.48 &0.00 &24.44 &0.02 &30.52 &0.08 \\
\textbf{Ours}& \textbf{52.70}& \textbf{0.30}& \textbf{48.05}& \textbf{0.25}& \textbf{34.00}& \textbf{0.01}& \textbf{56.68}& \textbf{0.37}&\textbf{44.97} & \textbf{0.20}\\

\bottomrule
\end{tabular}
}
\caption{The result of adding RAG module on Qwen2-72B-Instruct with different length sets. }
\label{tb:rag_qwen2}
\end{table*}

